Space-Aware Reconfiguration

We consider the problem of reconfiguring a set of physical objects into a desired target configuration, a typical (sub)task in robotics and automation, arising in product assembly, packaging, stocking store shelves, and more. In this paper we address a variant, which we call space-aware reconfiguration, where the goal is to minimize the physical space needed for the reconfiguration, while obeying constraints on the allowable collision-free motions of the objects. Since for given start and target configurations, reconfiguration may be impossible, we translate the entire target configuration rigidly into a location that admits a valid sequence of moves, where each object moves in turn just once, along a straight line, from its starting to its target location, so that the overall physical space required by the start, all intermediate, and target configurations for all the objects is minimized. We investigate two variants of space-aware reconfiguration for the often examined setting of $n$ unit discs in the plane, depending on whether the discs are distinguishable (labeled) or indistinguishable (unlabeled). For the labeled case, we propose a representation of size $O(n^4)$ of the space of all feasible initial rigid translations, and use it to find, in $O(n^6)$ time, a shortest valid translation, or one that minimizes the enclosing disc or axis-aligned rectangle of both the start and target configurations. For the significantly harder unlabeled case, we show that for almost every direction, there exists a translation in this direction that makes the problem feasible. We use this to devise heuristic solutions, where we optimize the translation under stricter notions of feasibility. We present an implementation of such a heuristic, which solves unlabeled instances with hundreds of discs in seconds.

==> chapters/sed3.tex <==
\section{Alternative Proof - Case(ii)}
I want to express a new algorithm for Case(iii) that better suits our $D_Q$ approach.
Fix $s_1, s_2 \in S$ (such that $s_1,s_2$ define an edge $e$ in $FVD(S)$) and $t_0 \in T$.
Assume wlog that the bisector $b(s_1,s_2)$ is the $x$-axis, the midpoint of $s_1$ and $s_2$ is the origin, and $t_0 = (0,0)$.
Also assume that we split $e$ in the origin and look on its positive direction to the right.
We are looking for a valid translation $\vec{v}$ such that the disc $D$ that $s_1,s_2,t_0$ lie on its boundary encloses $S$ and $T+\vec{v}$ and is size is minimized.
We say that a translation is enclosing, if the admitted disc is enclosing.
In order for $D$ to enclose $S$, it is enough to require that is center will lie on the edge $e$.
To satisfy this requirement, we limit $t_0 + \vec{v}$ (and so limiting $\vec{v}$) to be inside one of the following areas:
\begin{enumerate}[(1)]
	\item $\vec{v}_x > 0$, $\vec{v}$ is not in the open disc $D(\xi_1)$ and is inside the closed disc $D(\xi_2)$ (if exists); see Figure 8.
	\item $\vec{v}_x < 0$, $\vec{v}$ is inside the closed disc $D(\xi_1)$ and is outside the open disc $D(\xi_2)$ (if exists).
\end{enumerate}
We are left to enclose $T+\vec{v}$.
We can show that for each $t\in T\setminus\set{t_0}$ we get an hyperbola that together with the $y$-axis divides the translation plane into 6 areas, each in which either every translation is enclosing for $t$, or every translation is non-enclosing for $t$.
Observe that our goal here is to get $\vec{v}$ as close as possible (Euclidean distance wise) to the origin for $\vec{v}_x >0$, or farthest away from it for $\vec{v}_x < 0$.
We can thus observe that the translation we are looking for has to lie on one of the problems constraints: $D(\xi_1)$, $D(\xi_2)$, the $O(n)$ hyperbolas or $Q$.
For the first 3 constraints, we can create an arrangement of $O(n^2)$ size complexity. AND HERE IS THE PROBLEM! how can we even find the points for the first 3 constraints? and then on each vippodrome boundary?

We repeat the above process for every pair corresponding to the $O(n)$ edges of $FVD(S)$ and for every of the $O(n)$ points in $T$, which gives us $O(n^5 \log n)$ total running time for this case.

